A Feedback Capacity-Achieving Coding Scheme for the $(d,\infty)$-RLL Input-Constrained Binary Erasure Channel

This paper considers the memoryless input-constrained binary erasure channel (BEC). The channel input constraint is the $(d,\infty)$-runlength limited (RLL) constraint, which mandates that any pair of successive $1$s in the input sequence be separated by at least $d$ $0$s. We consider a scenario where there is causal, noiseless feedback from the decoder. We demonstrate a simple, labelling-based, zero-error feedback coding scheme, which we prove to be feedback capacity-achieving, and, as a by-product, obtain an explicit characterization of the feedback capacity. Our proof is based on showing that the rate of our feedback coding scheme equals an upper bound on the feedback capacity derived using the single-letter bounding techniques of Sabag et al. (2017). Further, we note using the tools of Thangaraj (2017) that there is a gap between the feedback and non-feedback capacities of the $(d,\infty)$-RLL input constrained BEC, at least for $d=1,2$.

==> BCJR_invar.tex <==
\label{subsec:BCJR_invar}

Given the $Q$-graph, $\mathscr{G}_Q^{(d)}$, for the $(d,\infty)$-RLL input constrained BEC, we call its corresponding $(S,Q)$ graph, $\mathscr{G}_{SQ}^{(d)}$, which is constructed following the description in definition \ref{def:SQ_graph}, with the presentation of channel states given in figure \ref{fig:d_inf_constraint}. 


%We note that our family of $(S,Q)$-graphs  possesses the following interesting property:
%
%\begin{proposition}\label{prop:lp}
%	In the setting of the $(d,\infty)$-RLL input-constrained BEC, for the $(S,Q)$-graphs, $\mathscr{G}_{SQ}^{(d)}$, we have that 
%	\begin{equation*}
%	\max_{\{{P}(x|s,v)\}} P(X=1)\leq \frac{1}{d+1},
%	\end{equation*}
%	where the maximum is taken over all input distributions, $\left({P}(\cdot|s,v): s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ such that the resulting Markov chain on $\mathscr{S}\times \mathscr{V}^{(d)}$ has a unique stationary distribution.
%\end{proposition}
%
%We prove Proposition \ref{prop:lp} by casting the maximization problem as a linear program (LP). We then use the weak duality theorem for LPs (see, for example, \cite{boyd}) to find a feasible point of the corresponding dual LP, the objective value at which serves as an upper bound for our maximization problem. The proof is dealt with in Appendix C.

In this subsection, we construct a BCJR-invariant input distribution, $\left(\left(\tilde{P}(x|s,v):x\in \mathscr{X}\right): (s,v)\in \mathscr{S}\times \mathscr{V}^{(d)}\right)$. In tandem, we will also identify the conditional distribution, $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$, for each $v\in \mathscr{V}^{(d)}$, where $\left(\tilde{\pi}(s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_{SQ}^{(d)}$
%, and $\tilde{\pi}(v) = \sum_{s\in \mathscr{S}}\tilde{\pi}(s,v)$.

%Before we do so, it will be useful to put down some additional notation. Now, for $\mathbf{q}\in \mathscr{V}^{(d)}$, let $(k_1^{\mathbf{q}},k_2^{\mathbf{q}},\ldots,k_{d+1}^{\mathbf{q}})$ denote the runlength sequence of $0$s and $?$s, in $\mathbf{q}$, defined as follows:

%If $\mathbf{q}$ begins with a run of $\ell$ $0$s, for $\ell \geq 1$, then $k_1^{\mathbf{q}} = \ell$; otherwise, $k_1^{\mathbf{q}} = 0$. Further, $k_2^{\mathbf{q}}$ is the length of the run of $?$s after the first run (if any) of $0$s; $k_3^{\mathbf{q}}$ is the length of the (second) run of $0$s after the first run of $?$s, and so on. 

%Note that $k_{2i-1}^{\mathbf{q}}$ records the length of a run of $0$s and $k_{2i}^{\mathbf{q}}$ records the length of a run of $?$s, for $i\geq 1$. Also, $k_{d+1}^{\mathbf{q}}\neq 0$ if, and only if, $\mathbf{q}$ is such that $q_{2i-1}=?$ and $q_{2i}=0$, for $i\geq 1$. Observe that $\sum_{i=1}^{d+1}k_i^{\mathbf{q}} = d$ and $k_i^{\mathbf{q}}\geq 0$, for all $i\in [d+1]$. We shall henceforth omit the superscript $\mathbf{q}$ since it will be apparent from the context.

Since our input distribution %$\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$,
must respect the $(d,\infty)$ input constraint, we need that $\tilde{P}(1|s,v)=0$, for $s\in \{0,1,\ldots,d-1\}$, and we hence need only specify $\tilde{P}(1|d,v)$, for each $v\in \mathscr{V}^{(d)}$, to completely determine the input distribution.

To this end, we first associate with every node $v\in \mathscr{V}^{(d)}$, a probability vector, $\boldsymbol{\theta}_v:=\left(\theta_v(s):s\in \mathscr{S}\right)$, of length $d+1$. 
%The vector $\boldsymbol{\theta}_v$ is a proxy for $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$ for a suitably defined input distribution.

We set $\boldsymbol{\theta}_{Q_i} = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. Further, in compliance with the $(d,\infty)$-RLL input constraint, we set $a_{Q_i}:=\tilde{P}(1|d,Q_i) = 0$, for $i\neq d$. Let us pick $a := \tilde{P}(1|d,Q_d)$, such that $a\leq \frac{1}{d+1}$. The reason for the restriction of $a$ to the interval $[0,\frac{1}{d+1}]$ will be made clear in Lemma \ref{lemma:domain}. 
%We shall, for conciseness of notation, represent $a_{Q_d}$ as $a$.

Now, for $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}^{(d)}_{\text{DB}}$, we define an accompanying vector $\boldsymbol{\beta}=(\beta_{0},\beta_{1},\ldots,\beta_{d-1})$, with\\ $\beta_s := |\{i\in [0:s-1]:w_i=0\}|$. In words, $\beta_s$ is the number of $0$s that appear strictly to the left of position $s$ in the $d$-tuple corresponding to $\mathbf{q}$. We then define $\boldsymbol{\theta}_{\mathbf{q}}$ as follows:

For $0\leq s\leq d-1$,
\begin{equation}\label{eq:theta_even}
{\theta}_{\mathbf{q}}(s) = 
\begin{cases}
0, & \text{ if } w_s=0,\\
\frac{a}{(1-a)^{\beta_s}}, & \text{ if }  w_s=\ ?,
\end{cases}
\end{equation}
and $\theta_{\mathbf{q}}(d) = 1-\sum_{s=0}^{d-1}\theta_{\mathbf{q}}(s)$. It is clear from our definition that $\boldsymbol{\theta}_{Q_d} = \mathbf{e}_{d}^{d}$, where $Q_d = (0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%If $d$ is odd, for $\mathbf{q} \in \mathscr{V}_{\text{DB}}^{(d)}$, we set
%\begin{equation}\label{eq:theta_odd}
%\theta_{\mathbf{q}}(s) = 
%\begin{cases}
%a, \ s\in [0:k_{d+1}-1],\\
%0, \ s\in [k_{d+1}:k_{d+1}+k_d-1],\\
%\frac{a}{(\bar{a})^{k_d}}, \ s\in [k_{d+1}+k_d:\sum\limits_{i\geq {d-1}}k_i -1],\\
%0, \ s\in [\sum\limits_{i\geq {d-1}}k_i:\sum\limits_{i\geq {d-2}}k_i-1],\\
%\quad \vdots\\
%\frac{a}{(\bar{a})^{\sum\limits_{i\geq 3: i\ \text{odd}}k_i}}, \ s\in [\sum\limits_{i\geq {3}}k_i:\sum\limits_{i\geq {2}}k_i],\\
%0, \ s\in [\sum\limits_{i\geq {2}}k_i:d-1],
%\end{cases}
%\end{equation}
%and $\theta_{\mathbf{q}}(d) = 1-\sum_{i=1}^{d-1}\theta_{\mathbf{q}}(i)$.

Finally, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, we let $a_{\mathbf{q}}:= \tilde{P}(1|d,\mathbf{q}) = \frac{a}{\theta_{\mathbf{q}}(d)}$. In order for $a_{\mathbf{q}}$ to be a valid probability, it must lie in $[0,1]$, a sufficient condition for which is provided by Lemma \ref{lemma:domain} below.

\begin{lemma}\label{lemma:domain}
	For $a\in [0,\frac{1}{d+1}]$, $a_{\mathbf{q}}\in [0,1]$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$ .
\end{lemma}

%The proof of this lemma is taken up in  Appendix A.
We refer the reader to \cite{fv} for the proof of the lemma above.
\begin{remark}
%Note that this procedure determines the vector $\left(a_v:v\in \mathscr{V}^{(d)}\right)$, thereby specifying the entire input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$.

Our input distribution is aperiodic for $a<\frac{1}{d+1}$ and $\epsilon\neq 1$, as then there exists a self-loop of positive probability, $\bar{a}\bar{\epsilon}$, from the node $(d,Q_d)$ to itself, in $\mathscr{G}_{SQ}^{(d)}$. The feedback capacity at $\epsilon=1$ is well-known to be $C^{\text{fb}}(1) = 0$, and we safely assume, going forward, that $\epsilon\neq 1$.
\end{remark}

%\begin{figure*}[t]
%	\centering
%	\subfloat[]{\includegraphics[width=0.2\linewidth]{1_inf.png}\label{fig:Q_1}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.4\linewidth]{2_inf.png}\label{fig:Q_2}}
%	\caption{The $Q$-graphs $\mathscr{G}^{(1)}_Q$ and $\mathscr{G}^{(2)}_Q$ are shown above in (a) and (b), respectively. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_1 = 0$, in $\mathscr{G}^{(1)}_Q$, and $Q_2 = (0,0)$, in $\mathscr{G}^{(2)}_Q$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%\end{figure*}
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.5]{2_inf_mod.png}
%	\caption{The $Q$-graph $\mathscr{G}^{(2)}_Q$ is shown above. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_2 = (0,0)$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%	\label{fig:Q_2}
%\end{figure}
%Before we set out to prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR invariant, we shall introduce one other piece of notation. For the function $B_s: \Delta(d)\times \mathscr{Y} \rightarrow \Delta(d)$ defined in equation \eqref{eq:bs}, we define the vector $\mathbf{B}(\mathbf{\theta_v},y)$ to be $\left(B_s(\mathbf{\theta_v},y): s\in \mathscr{S}, s\neq d\right)$, for $v\in \mathscr{V}^{(d)}$. For the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$, we can write down $\mathbf{B}(\mathbf{\theta_v},y)$ explicitly. For $v\in \mathscr{V}_{\text{DB}}^{(d)}$,

Before we prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR-invariant, we note that for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$, the value $B_s(\boldsymbol{\theta}_v,y)$ (see equation \eqref{eq:bs}) can be computed explicitly for the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$. 
%\begin{equation*}
%\mathbf{B}(\mathbf{\theta_v},y) = \begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\frac{\theta_{\mathbf{q}}(1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)}\right], \ y=0,\\
%\left[a_\mathbf{q}\theta_{\mathbf{q}}(d),\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation*}
%
For $0\leq s\leq d-1$, and for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, it holds that
\begin{equation}\label{eq:Bs0}
B_s(\boldsymbol{\theta}_\mathbf{q},y) = 
\begin{cases}
0, & \text{ if } s=0,\ y=0\\
\frac{\theta_{\mathbf{q}}(s-1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)} = \frac{\theta_{\mathbf{q}}(0)}{1-a}, & \text{ if } 1\leq s \leq d-1, \ y=0\\
a_\mathbf{q}\theta_{\mathbf{q}}(d) = a & \text{ if } s=0, \ y=?\\
\theta_{\mathbf{q}}(s-1), & \text{ if } 1\leq s \leq d-1, \ y=?\\
1, & \text{ if } s=0, \ y=1\\
0, & \text{ if } 1\leq s \leq d-1, \ y=1,
\end{cases}
\end{equation}
with $B_d(\boldsymbol{\theta}_\mathbf{q},y) = 1 - \sum_{s=0}^{d-1}B_s(\boldsymbol{\theta}_\mathbf{q},y)$, for $y\in \{0,?,1\}$. Note that the vector $\left(B_s(\boldsymbol{\theta}_\mathbf{q},1): s\in \mathscr{S}\right)$ is equal to $\mathbf{e}_0^{d}$.
%which results in
%\begin{equation}\label{eq:bs_BEC}
%\mathbf{B}(\mathbf{\theta_v},y) = 
%\begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a},\frac{\theta_{\mathbf{q}}(1)}{1-a},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a}\right], \ y=0,\\
%\left[a,\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation}
%since $a_\mathbf{q}\theta_{\mathbf{q}}(d)=a$.

Further, if $v=Q_i$, for some $i\in [0:d-1]$, it holds that
\begin{equation}\label{eq:BsQ}
\left(B_s(\boldsymbol{\theta}_v,y): s\in \mathscr{S}\right) = \mathbf{e}_{i+1}^{d},
\end{equation}
for $y\in \{0,?\}$.
%\begin{equation}\label{eq:bs_BEC_2}
%\mathbf{B}(\mathbf{\theta_v},y) = \mathbf{e}_{i+1}^{d},\ \text{for}\ y\in \{0,?\}.
%\end{equation} 
We now note that the following lemma holds:

\begin{lemma}\label{lemma:bcjr}
	The set of probability vectors $\left(\boldsymbol{\theta}_{v}: v\in \mathscr{V}^{(d)}\right)$ along with the input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ satisfies
	\begin{equation}\label{eq:bs_valid}
	\theta_{v^+}(s^+) = B_{s^+}(\boldsymbol{\theta}_v,y),
	\end{equation}
	for every $(s^+,v,y)\in \mathscr{S}\times \mathscr{V}^{(d)}\times \mathscr{Y}$, where $v^+ = \Phi(v,y)$, with $\Phi:\mathscr{V}^{(d)}\times \mathscr{Y}\rightarrow \mathscr{V}^{(d)}$ is the $Q$-node update function.
\end{lemma}
\begin{proof}
	If $v=Q_i$, for some $i\in [0:d-1]$, then, it follows from equation \eqref{eq:BsQ} that 	
	$\mathbf{e}_{i+1}^{d}=\left(B_s(\boldsymbol{\theta}_{Q_i},y):s\in \mathscr{S}\right)
	$ which, in turn, is equal to  $\boldsymbol{\theta}_{Q_{i+1}}$,	
	for $y\in \{0,?\}$. Equation \eqref{eq:bs_valid} then follows by noting that $\Phi(Q_i,y) = Q_{i+1}$, for $y\in \{0,?\}$.
	
	Now, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, when $y=1$, we see from equation \eqref{eq:Bs0} that	
	$\mathbf{e}_{0}^{d}=\left(B_s(\boldsymbol{\theta}_{v},1):s\in \mathscr{S}\right)$, which is equal to $\boldsymbol{\theta}_{Q_{0}}$.
	Since $\Phi(v,1) = Q_{0}$, it follows that equation \eqref{eq:bs_valid} holds.
	
	Now, let $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}_{\text{DB}}^{(d)}$. Then, since $\Phi(\mathbf{q},0) = (0,w_{0},w_{1},\ldots,w_{d-1}))=:\mathbf{q}_0^+$, and $\Phi(\mathbf{q},?) = (?,w_{0},w_{1},\ldots,w_{d-1})=:\mathbf{q}_?^+$,  we see from equations \eqref{eq:theta_even} and \eqref{eq:Bs0} that $\left(B_s(\boldsymbol{\theta}_\mathbf{q},0):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_0}$ and $\left(B_s(\boldsymbol{\theta}_\mathbf{q},?):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_?}$. Thus, equation \eqref{eq:bs_valid} holds in this case too.	
\end{proof}
We now define the joint distribution, $\theta(s,v):=\theta_v(s)\tilde{\pi}(v)$, where $\left(\tilde{\pi}(v):v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_Q^{(d)}$ induced by $\tilde{P}$. From Lemma \ref{lemma:bcjr} and from the lemma below, we get that $\tilde{P}$ is BCJR-invariant.

\begin{lemma}\label{lemma:stat_dist}
	It holds that $\theta(s,v) = \tilde{\pi}(s,v)$, for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$.
\end{lemma}
\begin{proof}
	Fix an $s^+ \in \mathscr{S}$, and a $v^{+}\in \mathscr{V}^{(d)}$. Now,
	\begin{align*}
	&\sum\limits_{s,v,x,y}\theta(s,v)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}\mathds{1}\{v^+=\Phi(v,y)\}\\
	&= \sum\limits_{v,y}\tilde{\pi}(v)\mathds{1}\{v^+=\Phi(v,y)\}\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\times\\
	&\quad \quad \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \mathds{1}\{s^+=f(x,s)\}\\
	&\stackrel{(a)}{=}\theta_{v^+}(s^+)\sum\limits_{v,y}\tilde{\pi}(v)P(y|v)\mathds{1}\{v^+=\Phi(v,y)\}\\
	&=\theta_{v^+}(s^+)\tilde{\pi}(v^+) = \theta(s^+,v^+),
	\end{align*}
	where (a) follows from Lemma \ref{lemma:bcjr}, since $\theta_{v^+}(s^+)P(y|q)=\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}$. Since this holds for all $(s^+,v^+) \in \mathscr{S}\times \mathscr{Y}$, it follows that $\theta(s^+,v^+) = \tilde{\pi}(s^+,v^+)$.
\end{proof}
The lemma above implies that $\boldsymbol{\theta}_v = \tilde{\pi}(\cdot|v)$, and using Lemma \ref{lemma:bcjr}, we can conclude that $\tilde{P}$ is BCJR-invariant.
\begin{remark}
	It can be shown that for a fixed value of $a$, there is a unique BCJR-invariant input distribution on $\mathscr{G}_{SQ}^{(d)}$. 
	%In particular, this means that for a fixed value of $a$, the probability\\ $P(Y=1|\mathbf{q}) = a\epsilon$, for all $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$.
\end{remark}

==> IEEETransactions_LaTeX/IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> IEEETransactions_LaTeX/Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Proof_UB.tex <==
\label{sec:proof_UB}
\begin{proof}
We shall compute the upper bound expression in theorem \ref{thm:UB} by considering the family of $Q$-graphs, $\mathcal{J}:=\{\hat{\mathscr{G}}_Q^{(d)}: d\in \mathbb{N}\}$, where $\hat{\mathscr{G}}_Q^{(d)}$ is shown in figure \ref{fig:G_hat} for some fixed $d$. Let $\hat{\mathscr{G}}_{SQ}^{(d)}$ denote the $(S,Q)$-graph corresponding to $\hat{\mathscr{G}}_Q^{(d)}$. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{UB_Q.png}
	\caption{The $Q$-graph, $\hat{\mathscr{G}}_Q^{(d)}$. The labels on the edges denote outputs.}
	\label{fig:G_hat}
\end{figure*}

It can be shown that the single closed communicating class in $\hat{\mathscr{G}}_{SQ}^{(d)}$ is precisely the collection $\{(i,\hat{Q}_i): i\in [0:d-1]\}\cup \{(s,\hat{Q}_d):s\in [0:d]\}$ of nodes. Further, since the inputs are constrained, it holds that $P(X=1|S=s,Q=\hat{q}) = 0$, for all $(s,\hat{q}) \neq (d,\hat{Q}_d)$, with $(s,\hat{q})$ in the closed class. Therefore, the matrix of conditional input distributions, $[P(x|s,\hat{q})]$, can be parameterized by a single parameter, $p:=P(X=1|S=d,Q=\hat{Q}_d)$.

A simple computation then reveals that the stationary distribution of nodes in the closed communicating class obey:
\begin{align*}
\pi(s,\hat{Q}_s) &= \frac{p\bar{\epsilon}}{1+dp}, \ s\in [0:d-1],\\
\pi(s,\hat{Q}_d) &= \frac{p\epsilon}{1+dp}, \ s\in [0:d-1], \\
\pi(d,\hat{Q}_d) &= \frac{1}{1+dp}.
\end{align*}
Further, it holds that the conditional probability,

\begin{align*}
P(Y=1|\hat{Q}_d) &= P(Y=1,X=1,S=d|\hat{Q}_d)\\
&=p\bar{\epsilon}\frac{\pi(d,\hat{Q}_d)}{\sum_{s=0}^{d}\pi(s,\hat{Q}_d)}\\
&= \frac{p\bar{\epsilon}}{1+dp\epsilon}.
\end{align*}

Then, by Theorem \ref{thm:UB}, it holds that
\begin{align*}
C_{(d,\infty)}^{\text{fb}} &\leq \sup_{P(x|s,q)\in \Omega} I(X;Y|Q)\\
&= \sup_{P(x|s,q)\in \Omega} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(a)}{=} \max_{p\in [0,1]} \bar{\epsilon}\left(\sum_{s=0}^{d}\pi(s,\hat{Q}_d)\right)h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&= \max_{p\in [0,1]} \frac{\bar{\epsilon}(1+dp\epsilon)}{1+dp}h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&\stackrel{(b)}{=} \max_{\delta \in [0,\frac{1}{1+d\epsilon}]} R(\delta),
\end{align*}
where, in (a), we have used the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$, and (b) follows by changing the variable used in the maximization to $\delta:= \frac{p}{1+dp\epsilon}$.

Now, we note that if $\epsilon^{\star}$ satisfies the equation
\[
(d\epsilon)^{\left(\frac{1}{1-\epsilon}+d\right)} = (1+d\epsilon)^d,
\]
then, the derivative evaluated at $\frac{1}{1+d\epsilon^{\star}}$,  $R^{\prime}\left(\frac{1}{1+d\epsilon^{\star}}\right)$, is equal to $0$. Further, from the proof of Corollaries \ref{coroll} in Appendix B, we observe that $R^{\prime}(\delta)$ is strictly decreasing in $\delta$, for $\delta\in [0,1]$. Hence, it follows that for $\epsilon>\epsilon^{\star}$, the derivative, $R^{\prime}\left(\frac{1}{1+d\epsilon}\right)>0$, with $R^{\prime}(0^+)>0$. 

Therefore, the non-causal capacity, which is a maximum over $[0,1]$ of $R(\delta)$, is strictly larger than the upper bound in Proposition \ref{lemma:UB}, for $\epsilon>\epsilon^{\star}$.
\end{proof}

==> Proof_main.tex <==
\label{sec:proof_thm}

\begin{proof}
For the $(d,\infty)$-RLL input-constrained BEC under the BCJR-invariant input distribution $\tilde{P}$ defined in subsection \ref{subsec:BCJR_invar}, we have that
\begin{align*}
I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(b)}{=} \bar{\epsilon}\sum_{v\in \mathscr{V}^{(d)}}\tilde{\pi}(v)h_b(P(X=1|v)) + h_b(\epsilon)- h_b(\epsilon)\\
&\stackrel{(c)}{=} \bar{\epsilon}\sum_{\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}}\tilde{\pi}(\mathbf{q})h_b(P(X=1|\mathbf{q}))\\
&\stackrel{(d)}{=}\bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
\end{align*}
where (a) follows from the fact that $H(Y|X,Q) = H(Y|X) = h_b(\epsilon)$, and (b) from the fact that $P(Y=?|v) = \epsilon$, for all $v\in \mathscr{V}^{(d)}$, with $P(Y=1|v) = \bar{\epsilon}P(X=1|v)$. We additionally use  the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$. Further, (c) holds since $P(X=1|Q_i) = 0$, for $i\in [0:d-1]$. To obtain the equality (d), note that for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$. Hence, from Lemma \ref{lemma:stat_dist}, it follows that that $P(X=1|\mathbf{q}) = a$.

%Now, since for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$, we get from Lemma \ref{lemma:stat_dist} that $P(X=1|\mathbf{q}) = a$. Hence, it follows that
%
%\begin{equation}\label{eq:I_eval}
%I(X;Y|Q) = \bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
%\end{equation}
Further, it is true that
\begin{align}\label{eq:stat_q}
1 &= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + \sum_{i=0}^{d-1}\tilde{\pi}(Q_i) \notag\\
&= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + d\tilde{\pi}(Q_0) \notag\\
&= (1+da\bar{\epsilon})\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}),
\end{align}
where the penultimate equality holds since $\tilde{\pi}(Q_0) = \tilde{\pi}(Q_i)$, for all $i\in [d-1]$. The last equality follows from the observation that $\tilde{\pi}(Q_0) = \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})P(Y=1|\mathbf{q}) = \bar{\epsilon}a\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})$.

Plugging \eqref{eq:stat_q} back into equation (d), we obtain that $I(X;Y|Q) = \frac{h_b(a)}{da+\frac{1}{1-\epsilon}}$, and taking a maximum over all \\$a\in [0,\frac{1}{d+1}]$, we get the required result.
\end{proof}



==> Q-construction.tex <==
\label{sec:Q_const}
%We shall henceforth consider $\mathscr{S} = \{0,1,\ldots,d\}$ to be the state alphabet, for the $(d,\infty)$-RLL input constrained BEC.
%
%
In this section, we shall construct a family of $Q$-graphs, indexed by $d$, and identify a BCJR-invariant input distribution on the $(S,Q)$-graph corresponding to each $Q$-graph in the family.

\subsection{Construction of Q-graphs}
\input{Q-graph_fly.tex}

\subsection{Construction of a BCJR-invariant input distribution}
\input{BCJR_invar.tex}

==> Q-graph_fly.tex <==
%First, we recall the definition of a De Bruijn graph.
%
%\begin{definition}
%	Given an alphabet $\Sigma = \{w_1,w_2,\ldots,w_m\}$, a $k$-dimensional De Bruijn graph $\mathscr{G}_{\text{DB}}^{(k)} = (\mathscr{V}_{\text{DB}}^{(k)},\mathscr{E}_{\text{DB}}^{(k)},\mathscr{L}_{\text{DB}}^{(k)})$ over $\Sigma$ is a labelled, directed graph with vertex set $\mathscr{V}_{\text{DB}}^{(k)}$, edge set $\mathscr{E}_{\text{DB}}^{(k)}$, and a labelling function $\mathscr{L}_{\text{DB}}^{(k)}: \mathscr{E}_{\text{DB}}^{(k)}\rightarrow \Sigma$. Each vertex $v\in \mathscr{V}$ can be uniquely identified by a $k$-tuple over $\Sigma$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(k)}$ can alternatively be written as $\mathbf{v} = (w_1^v,w_2^v,\ldots,w_k^v)$, where $w^v_i \in \Sigma$, for $i\in [k]$. Note that there are $m^k$ vertices in total.
%	
%	The edge set 	
%	\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(k)} = \lbrace\mathbf{e}:\mathbf{e} = &\left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right),\\
%	& \text{ for some $w_1^i,\ldots,w_k^i,w \in \Sigma$}\rbrace.
%	\end{align*}
%	
%	Further, for any edge \\$\mathbf{e} = \left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right)$, we write \\ $\mathscr{L}(\mathbf{e}) = w$.
%\end{definition}
With each value of $d$ corresponding to the $(d,\infty)$-RLL input-constrained BEC, we associate a $Q$-graph, $\mathscr{G}_{Q}^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, with vertex set $\mathscr{V}^{(d)}$, edge multi-set $\mathscr{E}^{(d)}$, and a labelling function $\mathscr{L}^{(d)}: \mathscr{E}^{(d)}\rightarrow \{0,?,1\}$.

We write $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0, Q_1,\ldots,Q_{d-1}\}$, where each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ is uniquely identified by a $d$-tuple over $\{0,?\}$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ can be written as $\mathbf{q} = (w_{0}^q,w_{1}^q,\ldots,w_{d-1}^q)$, where $w^q_i \in \{0,?\}$, for $i\in \{0,1,\ldots,d-1\}$. In what follows, we suppress the superscript $q$, as it will be clear from the context. Note that there are $2^d$ vertices in $\mathscr{V}_{\text{DB}}^{(d)}$. We denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.\footnote{The subscript ``DB'' indicates that the subgraph $\mathscr{G}_{\text{DB}}^{(d)} = (\mathscr{V}_{\text{DB}}^{(d)},\mathscr{E}_{\text{DB}}^{(d)},\mathscr{L}_{\text{DB}}^{(d)})$, of $\mathscr{G}_{Q}^{(d)}$, is a de Bruijn graph of order $d$, on $\{0,?\}$ symbols.}


We now construct the edge multi-set, $\mathscr{E}^{(d)}$. Firstly, for vertices in $\mathscr{V}_{\text{DB}}^{(d)}$, we define the set $\mathscr{E}_{\text{DB}}^{(d)}$ to consist of all edges $\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right)$, for $(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)}$. 
%\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(d)} = & \lbrace\mathbf{e}:\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right),\\
%	& \ \ \ \ \ \text{ for }(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)} \rbrace.
%\end{align*}
%
Further, for any edge $\mathbf{e} = \bigl((w_{0},w_{1}\ldots,w_{d-1})$, $(w,w_{0},w_{1},\ldots,w_{d-2})\bigr)$, we define the labelling function $\mathscr{L}_{\text{DB}}^{(d)}: \mathscr{E}_{\text{DB}}^{(d)}\rightarrow \{0,?\}$ such that $\mathscr{L}_{\text{DB}}^{(d)}(\mathbf{e}) = w$.

%In this discussion, we shall focus on $d$-dimensional De Bruijn graphs, $\mathscr{G}_{\text{DB}}^{(d)}$, over $\Sigma = \{0,?\}$. By the definition above, this is a graph with $2^d$ vertices, each identified by a unique $d$-tuple consisting of $0,?$ symbols. Let us denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%We construct the $Q$-graph, $\mathscr{G}_Q^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, where $\mathscr{E}^{(d)}$ is now taken to be a multi-set, by first adding $d$ additional vertices, $Q_0,Q_1,\ldots, Q_{d-1}$, to $\mathscr{V}_{\text{DB}}^{(d)}$. Hence, $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0,\ldots,Q_{d-1}\}$.

The edge set, $\mathscr{E}^{(d)}$, is constructed by adding to the set $\mathscr{E}_{\text{DB}}^{(d)}$, the edges $(\mathbf{q},Q_0)$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, and, corresponding to each $Q_i$, $i\in [0:d-1]$, two edges, $\mathbf{e}^{Q_i}_1$ and $\mathbf{e}^{Q_i}_2$, from $Q_i$ to $Q_{i+1}$. %Note that the $Q$-graph, $\mathscr{G}_Q^{(d)}$, has parallel edges. %which are precisely the edges from $Q_i$ to $Q_{i+1}$, for $i\in [0:d-1]$.

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=0.7\textwidth]{3_inf_LB_UB.png}
%	\caption{Plot comparing our lower bound with numerical evaluations of the upper bound from \cite{Graph_based}, for $d=3$.}
%	\label{fig:3_inf_compare}
%\end{figure*}



Finally, the labelling function, $\mathscr{L}^{(d)}:\mathscr{E}^{(d)}\rightarrow \{0,?,1\}$ is defined as:
\begin{equation}\label{eq:label}
\mathscr{L}^{(d)}(\mathbf{e})=
\begin{cases}
\mathscr{L}^{(d)}_{\text{DB}}(\mathbf{e}), & \text{ if } \mathbf{e}\in \mathscr{E}^{(d)}_{\text{DB}},\\
1, & \text{ if } \mathbf{e}=(\mathbf{q},Q_0) \text{ for } \mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}},\\
0 & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_1 \text{ for some } i\in [0:d-1],\\
? & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_2 \text{ for some } i\in [0:d-1].
\end{cases}
\end{equation}

%We note that $\mathscr{G}_Q^{(d)}$ satsifies the properties of a $Q$-graph detailed out in Section \ref{sec:Q-graph}. 
The $Q$-graph, $\mathscr{G}^{(1)}_Q$, is identical to the dynamic programming state diagram under the optimal policy, for the $(1,\infty)$-RLL input-constrained BEC \cite{SabBEC}. The $Q$-graph, $\mathscr{G}^{(2)}_Q$, is shown in Figure \ref{fig:Q_2}.

Our family of $Q$-graphs is then given by $\mathscr{H}:=\{\mathscr{G}^{(d)}_Q: d\in \mathbb{N}\}$, with the $Q$-graph $\mathscr{G}^{({d})}_Q$ being used to derive a lower bound for the $({d},\infty)$-RLL input-constrained BEC.
	
%\begin{remark}
%	The nodes $Q_0, Q_1,\ldots, Q_d$ of $\mathscr{G}^{(d)}_Q$ can be interpreted as follows. Let us define, for a fixed output sequence, $y^t$, the length-$(d+1)$ belief vector $\mathbf{z}_t:=\left(P(S_t=s_t|y^t):s_t\in \mathscr{S}\right)$. Note that the vector,  $\mathbf{z}_t$, which is an element of $\Delta(d)$, is precisely the state vector of the dynamic programming (DP) formulation of the feedback capacity problem \cite{Weiss}. The node $Q_i$ corresponds to the DP state $\mathbf{z}_t = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. This, in turn, has the interpretation that the nodes $Q_0,\ldots, Q_d$ represent the belief vectors when the decoder knows the channel state exactly.
%	
%%	Now, consider a node $\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}$, where $\mathbf{q}\in \{0,1\}^d$. Let $i_1,\ldots,i_k$, for $k\leq d$, denote the positions of the $?$ entries in in $\mathbf{q}$. We then interpret $\mathbf{q}$ as a proxy for the belief vector, $\mathbf{z}_t$, with non-zero entries in only the co-ordinates $d+1,d+1-i_1,\ldots,d+1-i_k$. Note that by our interpretation, $Q_d$, which represents the $d$-tuple $(0,\ldots,0)\in \mathscr{V}^{(d)}_{\text{DB}}$, corresponds to the belief vector $\mathbf{e}_{d+1}^{d+1}$, as described in the previous paragraph.
%\end{remark}




==> introduction.tex <==

Discrete memoryless channels (DMCs) were introduced by Shannon \cite{Sh48} as models for communication links, and have, since then, been the object of much research activity in information theory. It was shown by Shannon \cite{Sh56} that causal, noiseless feedback of the outputs does not increase the capacity of memoryless channels, which is given by $C = \sup_{P(x)}I(X;Y)$.


In this paper, we consider DMCs with input constraints, which are specific instances of discrete channels with memory, and which find application in magnetic and optical recording systems \cite{Roth}, \cite{Immink}. Such channels fall under the broad category of finite-state channels (or FSCs), the numerical computation of whose non-feedback capacities has been considered in works such as \cite{GBAA} and \cite{Han3}. Figure \ref{fig:genconstdmc} shows a generic DMC with input constraints, with causal, noiseless feedback. The computation of the feedback capacity of an FSC using a dynamic programming (DP) formulation first appeared in \cite{Chen} and was later extended in works such as \cite{Tatikonda1} and \cite{Tatikonda2}. In this work, we shall focus on the binary erasure channel (or BEC), the inputs of which are constrained to obey the $(d,\infty)$-runlength limited (RLL) input constraint\footnote{The $(d,\infty)$-RLL constraint is a special case of the $(d,k)$-RLL constraint on binary sequences, which requires that the length of any run of consecutive $0$s is at least $d$ and at most $k$.}, which mandates that there needs to be at least $d$ $0$s between any pair of successive $1$s. Such RLL input constraints are necessary for mitigating inter-symbol interference and timing and synchronization errors. As was shown in the works \cite{SabBEC}, \cite{Hanerasure}, and \cite{SabBIBO}, the capacities of the $(1,\infty)$-RLL input-constrained binary erasure and binary symmetric channels are strictly larger than their respective non-feedback capacities, for at least some values of the channel parameters, thereby demonstrating that for channels with memory, feedback may indeed increase capacity.

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.4]{genconstdmc.png}
	\caption{System model of an input-constrained DMC with causal, noiseless feedback.}
	\label{fig:genconstdmc}
\end{figure}

In the context of the BEC with input constraints, the feedback capacities of the $(1,\infty)$- and the $(0,k)$-RLL input constraints (for $k\geq 1$) were computed in the works \cite{SabBEC} and \cite{0k}, respectively. Both of these works put down an explicit coding scheme, whose rate equals the capacity of the BEC with non-causal knowledge of erasures\footnote{Informally, the non-causal capacity is the maximum achievable rate of a coding scheme for the BEC in a setting in which the encoder knows, \emph{prior} to the transmission of the $i^{\text{th}}$ bit $x_i$, whether or not $x_i$ will be erased.}, which, in turn, is as an upper bound on the feedback capacity. Interestingly, this gives rise to the fact that the non-causal capacities of the BEC with the $(1,\infty)$- and the $(0,k)$-RLL input constraints are equal to the respective feedback capacities. Moreover, it was shown in \cite{0k} that the feedback capacity of the $(2,\infty)$-RLL input-constrained BEC is less than the corresponding non-causal capacity, when the channel parameter, $\epsilon$, is equal to $0.5$. In this paper, we show that for the $(2,\infty)$-RLL input-constrained BEC, the feedback capacity is in fact equal to the non-causal capacity for $\epsilon\in [0,1-\frac{1}{2\log(3/2)}]$. This result is a by-product of the main theorem in our paper, which presents an analytical lower bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, for all $d$ greater than or equal to $1$. For the case when $d=1$, our lower bound is tight for all values of $\epsilon$ \cite{SabBEC}, and for $d=2$, our lower bound is numerically close to an upper bound derived using techniques in \cite{Graph_based}, for $\epsilon$ larger than $1-\frac{1}{2\log(3/2)}$, too. We also present analytical upper bounds on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, which, like our lower bounds, are single-parameter optimization problems. We observe that our bounds differ from the non-causal capacity expression (see \cite{0k}) in only the domain of maximization. 

Our techniques involve the use of the single-letter bounding techniques of Sabag et al. in \cite{Single}, and we come up with a specific $Q$-graph (or a $Q$-context mapping) and a choice of a specific ``BCJR-invariant'' input distribution, which gives rise to an achievable rate.

==> preamble.tex <==
% preamble.tex

\geometry{letterpaper, top=2.2in, headheight=1.7in}
\date{}

\makeatletter

\def\fulltitle#1{\def\@fulltitle{#1}}
\def\runningtitle#1{\def\@runningtitle{#1}}
\def\runningauthor#1{\def\@runningauthor{#1}}
\def\affiliation#1{\def\@affiliation{#1}}
\def\department#1{\def\@department{#1}}
\def\memoid#1{\def\@memoid{#1}}
\def\theyear#1{\def\@theyear{#1}}
\def\mydate#1{\def\@mydate{#1}}

\runningtitle{How to write an effective report} % Short title
\author{Your name \and John Doe \and Jane Doe} % Full list of authors
\runningauthor{Your name et al.} % Short list of authors
\affiliation{Your University} % Affiliation e.g. University or Company
\department{Your Department} % Department or Office
\memoid{AI Memo 777} % ID of the tech report
\theyear{2018} % year of the tech report
\mydate{August 08, 2018} %the date

\def\displaymydate{\@mydate}
\def\displaytheyear{\@theyear}
\def\displaymemoid{\@memoid}
\def\displaydepartment{\@department}
\def\displayaffiliation{\@affiliation}
\def\displayrunningauthor{\@runningauthor}
\def\displayrunningtitle{\@runningtitle}

\makeatother

\makeatletter
\patchcmd{\@zfancyhead}{\fancy@reset}{\f@nch@reset}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyorh}{\f@nch@orh}{}{}
\makeatother

% ----------
% fancyhdr setup
% ----------

\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}

\fancypagestyle{firstpage}
{
    \fancyhf{}
    \fancyhead{%
        \begin{center}
            \textsc{\displayaffiliation}\\
            \textsc{\displaydepartment}
        \end{center}
        \vspace*{0.5in}
        \displaymemoid
        \hfill
        \displaymydate
    }
    \fancyfoot[L]{\footnotesize \textbf{\textsc{\displayaffiliation} -- \displaytheyear}}
}
\fancyhead[EL]{\small \displayrunningauthor}
\fancyhead[ER]{\small Page \thepage}
\fancyhead[OL]{\small Page \thepage}
\fancyhead[OR]{\small \displayrunningtitle}

\chead{}
\lfoot{}
\cfoot{}
\rfoot{}

% ----------

\providecommand{\keywords}[1]{\noindent \textbf{Keywords:} #1} % keywords definition

\renewcommand{\familydefault}{\sfdefault} % sans-serif font
\setlength{\parskip}{1em} % 1em skip between paragraphs
\abslabeldelim{:} % use colon after the run-in 'Abstract' word
\setlength{\parindent}{0pt} % no indentantion for first page 
\setlength{\abstitleskip}{-\absparindent} % this is because the abstract package sets \absparindent to \parindent

\pretitle{\Large \begin{center}}
\posttitle{\\[2ex] \Large \textbf{by}\end{center}}

==> report_header.tex <==
\usepackage{ifthen}
\usepackage{cite}
\usepackage{algorithm}
\usepackage[cmex10]{amsmath} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)
\usepackage{amsthm,amsfonts,amssymb}
\usepackage[noend]{algpseudocode}
\setcounter{MaxMatrixCols}{17}

\usepackage{subfig}
\usepackage{blkarray}
\usepackage[mathscr]{euscript}
\usepackage{enumitem}
%\usepackage{romannum}
\usepackage{blkarray}
\usepackage{stfloats}%
%\newtheorem{theorem}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}[section]{Lemma}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
%\theoremstyle{definition}
%\newthorem{definition}{Definition}[section]
%\usetikzlibrary{graphs}
\usepackage{url}
\usepackage{arydshln}
\usepackage{mathtools}
\usepackage{dsfont}
%\usepackage{kbordermatrix}
%\newcommand{\indicator}[1]{\mathbb{1}_{\set{#1}}}
%\usepackage{braket}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)

\usepackage{geometry}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[runin]{abstract}
\usepackage{titling}
\usepackage{booktabs}
\usepackage{fancyhdr}
\usepackage{helvet}
\usepackage{csquotes}
\usepackage{graphicx}
\usepackage{blindtext}
\usepackage{parskip}
\usepackage{etoolbox}


==> rm.tex <==
\label{sec:rm}
In this section, we consider the BEC with the $(d,\infty)$-RLL input constraint, but in the absence of feedback. We first recall some well-known results on the capacity without feedback of general input-constrained DMCs.
\begin{theorem}[\cite{Gallager}, Chap. 4, \textsection 6]
	The capacity of an input-constrained DMC without feedback is given by:
	\[
	C_{\text{ic-DMC}} = \lim_{N\rightarrow \infty} \max_{P(x^N)}\frac{1}{N} I(X^N;Y^N),
	\]
	where the maximum is taken over input distributions, $\{P(x^N)\}$, which satisfy the input constraint.
\end{theorem}
The expression above is a multi-letter mutual information expression, the explicit computation of which is a well-known open problem. A common technique for lower bounding the capacity is the restriction of the input process to be a stationary and ergodic Markov process of finite order. This procedure is meaningful in the context of results such as those in \cite{chen} and \cite{litan}, which show that the capacity of any indecomposable FSC (of which input-constrained DMCs form a special class) can be approached arbitrarily closely by a sequence of stationary and ergodic Markov processes of increasing order. However, such results do not reveal insight into the capacity expression.

For the case when the input process is first-order Markov, some analytical lower bounds are known (see, for example, \cite{ZW88, Han2, arnk20, arnk21ncc}). We put down here the simplest of these results, which pertains to the input-constrained BEC with a $(d,k)$- or $(d,\infty)$-RLL input constraint.
\begin{lemma}[\cite{arnk20}, Theorems V.3 and V.4]
	\label{lem:linearlb}
	The capacity of the BEC with a $(d,k)$- or $(d,\infty)$-RLL input constraint is lower bounded as:
	\[
	C_{(d,k)}(\epsilon) \geq C_0^{(d,k)}\cdot (1-\epsilon);\quad C_{(d,\infty)}(\epsilon) \geq C_0^{(d,\infty)}\cdot (1-\epsilon).
	\]
\end{lemma}
However, the bounds above do not specify low-complexity encoding and decoding schemes that achieve the rates mentioned. Our objective is to identify explicit families of fixed-length codes that involve low complexity encoding and decoding procedures, and which achieve non-trivial rates over the $(d,\infty)$-RLL input-constrained BEC. As mentioned in Section \ref{sec:main}, we consider the Reed-Muller (RM) family of codes, $\{\mathcal{C}_m(R)\}$, which are such that any rate $R\in [0,1-\epsilon)$ is $(0,\infty)$-achievable (see Definition \ref{def:ach}) over the (unconstrained) BEC (see Theorem \ref{thm:kud1}). We then select subcodes that respect the $(d,\infty)$-RLL constraint, of such a capacity-achieving sequence of RM codes, and compute their rate. For notational convenience, we denote by $S_{(d,\infty)}^{(n)}$, the set of $n$-length binary vectors that respect the $(d,\infty)$-RLL constraint, i.e.,
\begin{align*}
S_{(d,\infty)}^{(n)}:=\bigl\{\mathbf{c} = (c_0,\ldots,c_{n-1}): \mathbf{c}\text{ respects the $(d,\infty)$-RLL} \text{ input constraint.}\bigr\}.
\end{align*}
Likewise,
\begin{align*}
	S_{(0,k)}^{(n)}:=\bigl\{\mathbf{c} = (c_0,\ldots,c_{n-1}): \mathbf{c}\text{ respects the $(0,k)$-RLL} \text{ input constraint.}\bigr\}.
\end{align*}
We suppress the superscript `$(n)$' if the length of the vector is clear from the context.

We begin with a simple observation, presented below as a lemma. We recall that the support of a vector $\mathbf{c}\in \mathbb{F}_2^{n}$,
\[
\text{supp}(\mathbf{c}) = \{i: c_i = 1\}.
\]

\begin{lemma}
	\label{lem:simplerm}
	Given $d\geq 1$, the vector $\mathbf{c}$ is such that $\mathbf{c}\in S_{(d,\infty)}$, if $\hat{\mathbf{c}}\in S_{(d,\infty)}$, and supp$(\mathbf{c}) \subseteq \text{supp}(\hat{\mathbf{c}})$.
\end{lemma}
\begin{proof}
	The proof is simply that if $\hat{\mathbf{c}}$ respects the $(d,\infty)$-RLL constraint, there are at least $d$ $0$s between successive $1$s, and since supp$(\mathbf{c}) \subseteq \text{supp}(\hat{\mathbf{c}})$, it is true that the same property holds for $\mathbf{c}$ as well.
\end{proof}
The proof of Theorem \ref{thm:rm} is given below. We use the convenient notation ${n\choose \leq k}$ to denote $\sum_{i=0}^{k}{n\choose i}$.

\begin{proof}
	For a fixed $d\geq 1$, let $z := \left \lceil \log_2(d+1)\right \rceil$. Consider the subcode $\mathcal{C}_m^{(d,\infty)}(R)$, of the code $\mathcal{C}_m(R)$, defined as:
	\begin{align*}
	\mathcal{C}_m^{(d,\infty)}(R):=\{\text{Eval}(f): f = \left(\prod_{i=m-z+1}^{m} x_i \right)\cdot g(x_{1},\ldots, x_{m-z}), \text{ where } \text{deg}(g)\leq r_m-z\}.
	\end{align*}
It is easy to verify that the polynomial $h(x_{m-z+1},\ldots,x_m):=\prod_{i=m-z+1}^{m} x_i$ is such that its corresponding evaluation vector, Eval$(h)$, obeys Eval$(h)\in S_{(d,\infty)}^{(2^m)}$. This is because Eval$_\mathbf{y}(h) = 1$ if, and only if, $(y_{m-z+1},\ldots,y_m) = (1,\ldots,1)$, and in the lexicographic ordering, such evaluation points $\mathbf{y}$ are spaced out by $2^z - 1$ points, where $2^z-1\geq d$. Hence, since for any polynomial $f$ such that $\text{Eval}(f)\in \mathcal{C}_m^{(d,\infty)}(R)$, it is true that supp$(\text{Eval}(f))\subseteq \text{supp}(\text{Eval}(h))$, it follows from Lemma \ref{lem:simplerm} that Eval$(f) \in S_{(d,\infty)}^{(2^m)}$. Therefore, for any $R\in (0,1)$, it holds that $\mathcal{C}_m^{(d,\infty)}(R)$ is a collection of RM codewords in $\mathcal{C}_m(R)$, all of which respect the input constraint.

By simple calculations, it follows that the rate of the subcode 
\begin{align}
	R_m^{(d,\infty)}&=\frac{\log_2(|\mathcal{C}_m^{(d,\infty)}|)}{2^m} \notag\\
		&= \frac{{m-z \choose \leq r_m-z}}{2^m}\notag\\
		& = \frac{1}{2^z} \cdot \frac{{m-z \choose \leq r_m-z}}{2^{m-z}}\notag\\
		&\xrightarrow[m \to \infty]{} 2^{-z}R. \label{eq:limrm1}
\end{align}
 To show that the limit in equation \eqref{eq:limrm1} indeed holds, we note that it is sufficient to show that the difference $|r_{m} - r_{m-z}|$ can be bounded above by a constant that does not depend on $m$. Indeed, it is true by our choice of $r_m$ that for large enough $m$,
\begin{align}
\label{eq:rmbound1}
	|r_m - r_{m-z}| &= \biggl| \frac{m}{2} + \frac{\sqrt{m}}{2}Q^{-1}(1-R) - 
	   \left(\frac{m-z}{2} + \frac{\sqrt{m-z}}{2}Q^{-1}(1-R)\right)\biggr| \notag\\
	&\leq \frac{z}{2}+\frac{\sqrt{z}}{2}\lvert Q^{-1}(1-R)\rvert
%	\begin{cases}
%		\frac{z}{2}, \ \text{if }R\leq 0.5,\\
%		\frac{z}{2}+\frac{\sqrt{z}}{2}Q^{-1}(1-R),\ \text{if %}R> 0.5.
%	\end{cases}
	%\left \lvert \frac{z}{2} + \frac{\sqrt{z}}{2}Q^{-1}(1-R) \right \rvert := \theta_d(R),
\end{align}
%and
%\begin{align}
%\label{eq:rmbound2}
%	|r_m - r_{m-z}| &=\biggl| \frac{m}{2} + \frac{\sqrt{m}}{2}Q^{-1}(1-R) - 
%	  \left(\frac{m-z}{2} + \frac{\sqrt{m-z}}{2}Q^{-1}(1-R)\right)\biggr| \notag\\
%	&\geq \frac{z}{2} := \gamma_d,
%\end{align}

\end{proof}
\begin{remark}
	We note, for example, when $d=1$, the rate calculated in Theorem \ref{thm:rm}, when using the sequence of codes $\{\mathcal{C}_m^{(d,\infty)}(1-\epsilon)\}$, is $\frac{1}{2}(1-\epsilon)$, which is less than the lower bound of $\approx 0.694\cdot(1-\epsilon)$, obtained from Lemma \ref{lem:linearlb}. However, we have identified, explicitly, a set of codewords that, when sent over an BEC, can be decoded using low-complexity decoders for RM codes (see, for example, \cite{rm_survey}).
\end{remark}
\begin{remark}
	The achievable rate calculated in this paper supplements the results of \cite{pvk}, which, when suitably modified, show the existence of $(d,\infty)$-RLL subcodes of cosets of any $(0,\infty)$-capacity-achieving linear code, of rate at least $C_0^{(d,\infty)} - \epsilon$. We note in addition that our achievable rate exceeds the lower bound in \cite{pvk}, for large $\epsilon$.
\end{remark}
The proof of Theorem \ref{thm:0k} is similar to that of Theorem \ref{thm:rm}, and is stated below.
\begin{proof}
    For a fixed $k\geq 1$, let $t:= \left \lfloor \log_2(k+1)\right \rfloor$. Consider the subcode $\mathcal{C}_m^{(0,k)}(R)$, of the code $\mathcal{C}_m(R)$, defined as:
	\begin{align}
	\label{eq:0kconst}
	\mathcal{C}_m^{(0,k)}(R):=\{\text{Eval}(f)&: f = 1+(1+x_S)\cdot g(x_{1},\ldots, x_{m-t}),  \notag\\ &\text{ where }S\neq \emptyset, S \subseteq [m-t+1:m], \text{ and }\text{deg}(g)\leq r_m-|S|\}.
	\end{align}
	It can be checked that $\mathcal{C}_m^{(0,k)}(R)$ consists of only codewords $\mathbf{c}\in S_{(0,k)}^{(2^m)}$, via Lemma \ref{lem:simplerm}, and using the fact that Eval$(x_S)$ has runs of $0$s of length at most $2^t$, for $S$ as in \eqref{eq:0kconst}. It then holds that Eval$((1+x_S))$ has runs of $1$s of length at most $2^t$, and since supp$(\text{Eval}((1+x_S)g))\subseteq \text{supp}(\text{Eval}(1+x_S))$, the desired property of Eval$(f)$ readily follows. 
	
	Again, by simple calculations, it follows that the rate of the subcode
	\begin{align}
	R_m^{(0,k)}&=\frac{\log_2(|\mathcal{C}_m^{(0,k)}|)}{2^m} \notag\\
		&\stackrel{(a)}{\geq} \frac{\log_2\left(2^t\cdot \text{exp}_2\left({m-t \choose \leq r_m-t}\right)\right)}{2^m}\notag\\
		& = \frac{1}{2^t} \cdot \frac{t+{m-t \choose \leq r_m-t}}{2^{m-t}}\notag\\
		&\xrightarrow[m \to \infty]{} 2^{-t}R, \notag
\end{align}
where (a) follows from the fact that for each of the $2^t$ non-empty subsets $S\subseteq[m-t+1:m]$, there are at least $\text{exp}_2\left({m-t \choose \leq r_m-t}\right)$ polynomials $g(x_1,\ldots,x_{m-t})$, having degree at most $r_m-t$. Further, the limit in the last step follows from the arguments in equation \eqref{eq:rmbound1}.% and \eqref{eq:rmbound2}.
\end{proof}
It would be remiss to not comment on the rates achieved by polar codes over our class of $(d,\infty)$-RLL input-constrained erasure channels, given that polar codes are capacity-achieving over a broad class of channels (see, for example, \cite{polar}, \cite{tal}, \cite{tal2}, and reference therein). Following the work of Li and Tan in \cite{litan} and as pointed out earlier, it holds that the capacity without feedback of our class of channels can be approached arbitrarily closely using stationary, ergodic Markov input distributions of finite order. Moreover, it was shown in \cite{tal} that polar codes do achieve the information rates over the BEC, of any stationary, ergodic Markov input process, thereby showing that polar codes do achieve the capacity of our class of channels as well. However, this observation is not very helpful for the following reasons:
\begin{itemize}
	\item We do not possess knowledge of an optimal sequence of Markovian input distributions.
	\item Polar codes are (structured) random codes, and the exact choice of the bit-channels to send information bits over, requires analysis. In our construction, however, we have explicitly identified the codewords being transmitted.
	\item Finally, this observation does not lend insight into explicit lower bounds on non-feedback capacity.
\end{itemize}

==> rmub.tex <==
\label{sec:rmub}
In this section, we provide upper bounds on the rates over the $(1,\infty)$-RLL input-constrained BEC, achievable using subcodes of any $(0,\infty)$-capacity-achieving (over the unconstrained BEC) family of RM codes, under the standard lexicographic ordering. %For simplicity, we first present the analysis for the case when $d=1$, and extend the arguments to general $d$, later.

Following the expositions in \cite[Chap. 13]{mws} and \cite{rm_survey}, it holds that any Boolean polynomial $f \in \mathbb{F}_2[x_1,\ldots,x_m]$, such that Eval$(f) \in \text{RM}(m,r)$, can be expressed as:
\begin{equation}
	\label{eq:rmdecomp}
f(x_1,\ldots,x_m) = g(x_1,\ldots,x_{m-1}) + x_m\cdot h(x_1,\ldots,x_{m-1}), 
\end{equation}
where $g,h$ are such that Eval$(g)\in \text{RM}(m-1,r)$ and Eval$(h)\in \text{RM}(m-1,r-1)$. The following lemma then holds true:
\begin{lemma}
	\label{lem:necesscond}
	If a codeword Eval$(f)\in \text{RM}(m,r)$ is such that Eval$(f)\in S_{(1,\infty)}$, then, supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$, where $g,h$ are as in \eqref{eq:rmdecomp}.
\end{lemma}
\begin{proof}
	Suppose that there exists some evaluation point $\mathbf{z} = (z_1,\ldots,z_{m-1}) \in \mathbb{F}_2^{m-1}$ such that $g(\mathbf{z})=1$ and $h(\mathbf{z})=0$. Then it follows that at evaluation points $\mathbf{z}_1,\mathbf{z}_2 \in \mathbb{F}_2^m$ such that $\mathbf{z}_1 = \mathbf{z}0$ and $\mathbf{z}_1 = \mathbf{z}1$, it holds that $f(\mathbf{z}_1) = f(\mathbf{z}_2) = 1$. Since by construction the points $\mathbf{z}_1$ and $\mathbf{z}_2$ are consecutive in the lexicographic ordering, the codeword Eval$(f)\notin S_{(1,\infty)}$. 
\end{proof}
%\begin{remark}
%	In fact, a simple, sufficient condition can also be derived for Eval$(f)\in \text{RM}(m,r)$ to respect the $(1,\infty)$-RLL constraint, by requiring that $h$ take on the value of $1$ at points just prior to the start of a run of $1$s in Eval$(g)$. However, since this condition is not required for the upper bounding technique, we omit a detailed description. 
%\end{remark}
Now consider any sequence of RM codes, $\{{\mathcal{C}}_m(R)\}$, where ${\mathcal{C}}_m(R) = \text{RM}(m,r_m)$, where $r_m$ is as in \eqref{eq:rmval}. By Theorem \ref{thm:kud1}, we know that the sequence $\{\mathcal{C}_m(R)\}$ achieves a rate of $R\in (0,1-\epsilon)$ over the unconstrained BEC. From Lemma \ref{lem:necesscond}, it follows that in order to obtain an upper bound on the number of codewords, Eval$(f) \in {\mathcal{C}}_m(R)$, that respect the $(1,\infty)$-RLL constraint, it is sufficient to obtain an upper bound on the number of polynomials $h$, for a given $g$, such that supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$.

The following two lemmas from the literature will be useful in the proof of Theorem \ref{thm:rmub}.
\begin{lemma}[\cite{rm_survey}, Lemma 36]
	\label{lem:short}
	Let $\mathcal{V} \subseteq \mathbb{F}_2^m$ be such that $|\mathcal{V}|\geq 2^{m-u}$, for some $u\in \mathbb{N}$. Then, it holds that
	\[
	\text{rank}(G(m,r)[\mathcal{V}])> {m-u \choose \leq r},
	\]
	where $G(m,r)$ is the generator matrix of the RM$(m,r)$ code, and $G(m,r)[\mathcal{V}]$ denotes the set of columns of $G(m,r)$, indexed by $\mathcal{V}$.
\end{lemma}
\begin{lemma}[\cite{sam}, Proposition~1.6]
	\label{lem:sam}
	Let $\mathcal{C}^{\prime}_n$, of block length $n$ and rate $R^{\prime}=R(\mathcal{C}^{\prime}_n)$, be the dual of a linear code $\mathcal{C}_n$, of rate $R(\mathcal{C}_n)$, such that $\{\mathcal{C}_n\}$ achieves the rate $R = \lim_{n\to \infty} R(\mathcal{C}_n)$ over the unconstrained BEC. Let $\left(A_{\mathcal{C}^{\prime}_n}(w): 0\leq w\leq n\right)$ be the weight distribution of $\mathcal{C}^{\prime}_n$. Then, it holds that
	\[
	A_{\mathcal{C}^{\prime}_n}(w)\leq 2^{o(n)}\cdot\left(\frac{1}{1-R^{\prime}}\right)^{(2\ln2)w},
	\]
	where $o(n)$ denotes a term $a_n$ such that $\lim_{n\to \infty}\frac{a_n}{n} = 0$.
\end{lemma}
We now proceed to a proof of Theorem \ref{thm:rmub}.
\begin{proof}
	Fix the sequence $\{{\mathcal{C}}_m(R) = \text{RM}(m,r_m)\}$ of RM codes, with
	\[
		r_m = \max \left\{\left \lfloor \frac{m}{2}+\frac{\sqrt{m}}{2}Q^{-1}(1-R)\right \rfloor,0\right\},
	\]
	where $R\in (0,R^*)$, for $R^*$ as in the statement of the theorem.
	As explained in the discussion, any Boolean polynomial $f$ whose evaluation Eval$(f)\in \hat{\mathcal{C}}_m$ can be expressed as
	\[
	f(x_1,\ldots,x_m) = g(x_1,\ldots,x_{m-1}) + x_m\cdot h(x_1,\ldots,x_{m-1}), 
	\]
	where $g,h$ are such that Eval$(g)\in \text{RM}(m-1,r)$ and Eval$(h)\in \text{RM}(m-1,r-1)$. Now, for any codeword Eval$(g) \in \text{RM}(m-1,r_m)$ of weight $w$, we shall first calculate the number, $N_w(g)$, of codewords Eval$(h) \in \text{RM}(m-1,r_m)$ such that supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$. Note that $N_w(g)$ serves as an upper bound on the number of codewords Eval$(h) \in \text{RM}(m-1,r_m-1)$ such that the same property holds.
	
	To this end, suppose that wt$(\text{Eval}(g)) = w \geq2^{m-1-u}$. Note that for any polynomial $g$ as above of weight $w$, the number of codewords in the code produced by shortening RM$(m-1,r_m-1)$ at the indices in supp$(\text{Eval}(g))$ indeed equals $N_w(g)$. Now, since dim$(\text{RM}(m-1,r_m)) = {m-1\choose \leq r_m}$, and from the fact that $w\geq 2^{m-1-u}$, we obtain by an application of Lemma \ref{lem:short} and the rank-nullity theorem, that
	\begin{equation}
		\label{eq:nw}
	N_w(g)\leq \text{exp}_2\left({m-1\choose \leq r_m} - {m-1-u \choose \leq r_m}\right).
	\end{equation}
	Note that the right-hand side depends on the polynomial $g$ only via a lower bound on its weight $w$. We thus write $N_w(g)$ as simply $N_w$.
	
	Let $\mathsf{R}_{{\mathcal{C}},m}^{(1,\infty)}(R)$ be the rate of the largest $(1,\infty)$-subcode of ${\mathcal{C}}_m(R)$, i.e.,
	\[
	\mathsf{R}_{{\mathcal{C}},m}^{(1,\infty)}(R) = \frac{\log_2(|\mathcal{H}_{(1,\infty)}^{(m)}|)}{2^m},
	\]
	where we let $\mathcal{H}_{(1,\infty)}^{(m)}$ denote the largest $(1,\infty)$-subcode of ${\mathcal{C}}_m(R)$. Then, it holds that
	\begin{align}
|\mathcal{H}_{(1,\infty)}^{(m)}|&\leq \sum_{g: \text{Eval}(g)\in \text{RM}(m-1,r_m)}{N_w(g)}\\
		&\stackrel{(a)}{=} \sum\limits_{w=2^{m-1-r_m}}^{2^{m-1}}A_{m-1,r_m}(w){N_w} \notag\\
		&\stackrel{(b)}{<} \left\{\sum\limits_{w=2^{m-1-r_m}}^{2^{m-2}}A(w){N_w}\right\}+\frac{1}{2}.\text{exp}_2\left(m-1\choose \leq r_m\right)\times
		\text{exp}_2\left({m-1\choose \leq r_m} - {m-2\choose \leq r_{m}}\right)\notag \\
		&\stackrel{(c)}{<} \left\{\sum\limits_{w=2^{m-1-r_m}}^{2^{m-2}}A(w){N_w}\right\}+
		\frac{1}{2}\cdot\text{exp}_2\left({m-1\choose \leq r_m}+{m-2\choose \leq r_{m}}\right)\notag\\
		&\stackrel{(d)}{\leq} \Bigg\{\sum\limits_{i=1}^{{r_m-1}}A([2^{m-2-i}: 2^{m-1-i}])\times
		 \text{exp}_2\left({m-1\choose \leq r_m} - {m-2-i \choose \leq r_m}\right)\Bigg\}+
		 \frac{1}{2}\cdot\text{exp}_2\left({m-1\choose \leq r_m}+{m-2\choose \leq r_{m}}\right) \label{eq:sub1},
	\end{align}
where $A([a:b])$ is short for $\sum_{i=a}^{b}A(w)$. Here,
\begin{enumerate}[label = (\alph*)]
	\item follows from the observation that $N_w(g)$ depends only the weight $w$ of Eval$(g)$,
	\item holds due to the following fact: since the all-ones codeword $\mathbf{1}$ is present in RM$(m-1,r_m)$, it implies that $A_{m-1,r_m}(w) = A(w) = A(2^{m-1}-w)$, i.e., that the weight distribution of codewords is symmetric about weight $w=2^{m-2}$. Therefore,
	\begin{equation}
		\label{eq:Aw}
		A(w>2^{m-2})\leq \frac{1}{2}.\text{exp}_2\left(m-1\choose \leq r_m\right).
	\end{equation}
	The strict inequality in (b) follows from the observation that the codeword Eval$(x_m)\in \text{RM}(m-1,r_m)$, for $m\geq 2$, and that wt$(\text{Eval}(x_m)) = 2^{m-2}$. 
	\item follows from Pascal's rule in combinatorics that for any $n,k \in \mathbb{N}$ with $n>k$:
	\[
	{n-1\choose k}+{n-1\choose k-1} = {n\choose k}.
	\]
	Picking $n=m-1$ and $k=r_m$, we obtain that
	\[
	{m-1\choose r_m}-{m-2\choose r_m} = {m-2\choose r_m-1},
	\]
	and hence that
	\[
	{m-1\choose \leq r_m}-{m-2\choose \leq r_m} < {m-2\choose \leq r_m}.
	\]
	\item holds from equation \eqref{eq:nw}.
\end{enumerate}
It is clear that a simplification of equation (d) depends crucially on good upper bounds on the weight distribution function. Now, since the code RM$(m-1,r_m)$ is obtained by shortening the code RM$(m,r_m)$ at positions $\mathbf{z} = (z_1,\ldots,z_m)$ where $z_m=1$, we obtain that $A_{m-1,r_m}(w)\leq A_{m,r_m}(w)$. Note that the sequence of codes $\{{\mathcal{C}}_m(R) =\text{RM}(m,r_m)\}_{m\geq 1}$ is such that the sequence of dual codes $\{\text{RM}(m,m-r_m-1)\}_{m\geq 1}$ (see, for example, \cite{mws}) achieves a rate $1-R$ over the unconstrained BEC, we can use the result in Lemma \ref{lem:sam}.

Now, we use Lemma \ref{lem:sam} to get that
\begin{align}
	A_{m-1,r_m}([2^{m-2-i}: 2^{m-1-i}])&\leq A_{m,r_m}([2^{m-2-i}: 2^{m-1-i}])\\ &\leq 2^{o(2^m)}\cdot \sum_{w=2^{m-2-i}}^{2^{m-1-i}}2^{\left(2\ln 2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot w\right)} \notag\\
	&<  2^{o(2^m)}\cdot\sum_{w=2^{m-2-i}}^{2^{m-1-i}}2^{2\ln 2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot w} \notag\\
	&<  \text{exp}_2\left(2\ln 2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i}+o(2^m)\right) \notag\\
	&= 2^{o(2^m)}\cdot \text{exp}_2\left(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i}\right). \label{eq:sub2}
\end{align}
Therefore, putting \eqref{eq:sub2} back in \eqref{eq:sub1}, we get that
\begin{align}
	2^m\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R) &= \log_2|\mathcal{H}_{(1,\infty)}^{(m)}| \notag\\
	&< {m-1 \choose \leq v_m}+{m-2 \choose \leq v_m}+ 
	 \log_2\Bigg\{\frac{1}{2}+2^{o(2^m)}\cdot \Bigg[\sum_{i=1}^{r_m-1}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right) \cdot 2^{m-1-i} - 
	  {m-2-i \choose \leq r_m} - {m-2 \choose \leq v_m}\Bigg)\Bigg]\Bigg\} \notag\\
	  &<{m-1 \choose \leq r_m}+{m-2 \choose \leq v_m}+
	  \log_2\Bigg\{2.2^{o(2^m)}\cdot \Bigg[\sum_{i=1}^{r_m-1}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i} - 
	  {m-2-i \choose \leq r_m}-{m-2 \choose \leq v_m}\Bigg)\Bigg]\Bigg\} \notag\\
	  &= {m-1 \choose \leq r_m}+ o(2^m) +
	  \log_2\Bigg\{\sum_{i=1}^{r_m-1}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i} - 
	  {m-2-i \choose \leq r_m}\Bigg)\Bigg\} \label{eq:subs3}
\end{align}
Let $\gamma:= -Q^{-1}(1-R)>0$, since $R\in (0,R^*)$, where $R^*<0.5$. Now, note that for $z<m$, and for $m$ large enough, it holds by our choice of $r_m$ that:
\begin{align*}
r_m - r_{m-z} &= \left(\frac{m}{2}-\frac{\gamma \sqrt{m}}{2}\right)-\left(\frac{m-z}{2}-\frac{\gamma \sqrt{m-z}}{2}\right)\\
&\geq\frac{z}{2}-\frac{\gamma \sqrt{z}}{2}
\geq 0,
\end{align*}
for $z\geq \gamma^2$. Therefore, for $m$ large enough and for $i\in [\gamma^2-2:r_m-1]$, it holds that the term 
\begin{align}
\label{eq:subs1}
{m-2-i \choose \leq r_m} > {m-2-i \choose \leq r_{m-2-i}}. 
\end{align}

Furthermore, for $i\in [1:\gamma^2-3]$, from equation \eqref{eq:rmbound1}, we see that
\[
r_m \geq r_{m-2-i}-\left(\frac{i+2+\gamma\sqrt{i+2}}{2}\right).
\]
This then implies that for $i\in [1:\gamma^2-3]$,
\begin{align}
{m-2-i \choose \leq r_m}\geq {m-2-i \choose \leq r_{m-2-i}} - \frac{i+2}{2}\cdot {m-2-i\choose \frac{m-2-i}{2}} \notag\\
\geq {m-2-i \choose \leq r_{m-2-i}} - \frac{\gamma^2-1+\gamma\sqrt{\gamma^2-1}}{2}\cdot {m-2-i\choose \frac{m-2-i}{2}} \label{eq:subs2}.
\end{align}
Plugging equations \eqref{eq:subs1} and \eqref{eq:subs2} into \eqref{eq:subs3}, we get that
\begin{align}
	2^m\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R)&<{m-1 \choose \leq r_m}+ o(2^m) +
	\log_2\Bigg\{\sum_{i=1}^{\gamma^2-3}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i} - \notag\\
	&\ \ \ \ \ {m-2-i \choose \leq r_{m-2-i}}+\frac{\gamma^2-1+\gamma\sqrt{\gamma^2-1}}{2}\cdot {m-2-i \choose \frac{m-2-i}{2}}\Bigg) + \sum_{i=\gamma^2-2}^{r_m-1}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i} - 
	{m-2-i \choose \leq r_{m-2-i}}\Bigg)\Bigg\}\notag\\
	&< {m-1 \choose \leq r_m}+ o(2^m) +
	\log_2\Bigg\{\text{exp}_2\left(\frac{\gamma^2-1+\gamma\sqrt{\gamma^2-1}}{2}\cdot {m-3 \choose \frac{m-3}{2}}\right)\times \notag\\
	&\ \ \ \ \ \ \ \ \ \ \ \ \ \sum_{i=1}^{r_m-1}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i} - 
	{m-2-i \choose \leq r_{m-2-i}}\Bigg)\Bigg\} \label{eq:subs}
\end{align}
%\textbf{Unsure how to proceed. Ask sir. What we'd like to show is:}\\
%\textbf{\textbackslash begin}
Now, observe that for any $\delta>0$ and for $m>m_0(\delta)$, with $i\in [1:r_m-1]$, it holds that
\[
\frac{{m-2-i \choose \leq r_{m-2-i}}}{2^m}\geq (1 - \delta)\cdot \frac{R}{2^{i+2}},
\]
%Further, it is possible to pick a subsequence $\{m_k\}_{k\geq 1}$, such that $m_k\to \infty$ as $k\to \infty$, such that for fixed $\delta_i$, where $i\in [1:r_m-1]$, it holds that
%\[
%\frac{{m_k-2-i \choose \leq r_{m_k-2-i}}}{2^{m_k}}\geq \frac{R}{2^{i+2}} - \frac{\delta_i}{2^{m_k}},
%\]
or, equivalently, that
\begin{equation}
\label{eq:doubt}
{m-2-i \choose \leq r_{m-2-i}}\geq (1-\delta)\cdot 2^{{m}-i-2}\cdot R
\end{equation}
Substituting equation \eqref{eq:doubt} back in \eqref{eq:subs}, we see that by letting $m\to \infty$, % along the subsequence $\{m_k\}_{k\geq 1}$,
\begin{align}
	{R}^{(1,\infty)}_{{\mathcal{C}}}(R) &= \lim_{m\to \infty}\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R)\notag\\
	&<\lim_{m\to \infty} \frac{1}{2^m}\Bigg[{m-1 \choose \leq r_m}+ o(2^m) + \frac{\gamma^2-1+\gamma\sqrt{\gamma^2-1}}{2}\cdot {m-3 \choose \frac{m-3}{2}}+
	\log_2\Bigg\{\sum_{i=1}^{r_m-1}\text{exp}_2\Bigg(2\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i} - \\ 
	& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 2^{{m}-i-2}\cdot R(1-\delta)\Bigg)\Bigg\}\Bigg]\notag\\
	&\stackrel{(a)}{=} \frac{R}{2} + \lim_{m\to \infty} \frac{1}{2^m}\log_2\Bigg\{\sum_{i=1}^{r_m-1}\text{exp}_2\Bigg(2^{{m}-i-2}\left[4\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)  - 
	R(1-\delta)\right] \Bigg)\Bigg\}\notag\\
	&\leq \frac{R}{2} + \lim_{m\to \infty} \frac{1}{2^m}\log_2\Bigg\{(r_m-1)\cdot\text{exp}_2\Bigg( 2^{m-3}\left[4\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)  - 
	R(1-\delta)\right]\Bigg)\Bigg\}\notag\\
	&= \frac{R}{2}+\frac{4\ln2\cdot\log_2 \left(\frac{1}{1-R}\right)  - 
		R(1-\delta)}{8} \notag\\
	&= \frac{3R}{8}+\frac{1}{2}\ln \left(\frac{1}{1-R}\right)+\frac{R\delta}{8}\label{eq:doubt2}.
\end{align}
Note that equation (a) above holds by the facts that ${m-3 \choose \frac{m-3}{2}} = o(2^m)$ and that $\lim_{m\to \infty} \frac{{m-1 \choose \leq r_m}}{2^m} = \frac{R}{2}$, following the arguments in equation \eqref{eq:rmbound1}. Since equation \eqref{eq:doubt2} holds for all $\delta>0$, we can let $\delta\to 0$, thereby obtaining that
\begin{align}
\label{eq:doubtf}
{R}^{(1,\infty)}_{{\mathcal{C}}}(R) \le \frac{3R}{8}+\frac{1}{2}\ln \left(\frac{1}{1-R}\right).
\end{align}
It can be numerically verified that for $R\in (0,R^*)$, where $R^*$ is as in the statement of the theorem, it holds that the right-hand side of equation \eqref{eq:doubtf} is less than $R$, thereby providing a non-trivial upper bound. Finally, we note that since $|\mathcal{H}_{(1,\infty)}^{(m)}|\leq |\mathcal{C}_m(R)|$, the trivial upper bound of ${R}^{(1,\infty)}_{{\mathcal{C}}}(R)\leq R$ holds for all $R\in (0,1)$.
%\textbf{\textbackslash end}
\end{proof}
%\begin{align}
%	\mathsf{R}_{(1,\infty)}^{\text{RM}} &= \lim_{m\to \infty} \mathscr{R}_{(1,\infty)}^{(m)} \notag\\
%	&< \lim_{m\to \infty} \frac{{m-1 \choose \leq v_m}+{m-2\choose \leq v_m}}{2^m} \notag\\
%	&= \frac{3R}{4}, \label{eq:append}
%\end{align}
%where the proof of equation \eqref{eq:append} is postponed to Appendix B. The proof follows along similar lines as the last part of the proof of Theorem \ref{thm:rm}, but crucially employs the assumption that $R<0.5$. Since the arguments must hold for any capacity-achieving (over the unconstrained BEC) sequence of RM codes, a more careful bounding technique is required.
%\end{proof}
%
%Note that we have only as yet proved an upper bound for the special case when $d=1$. However, before we generalize the arguments to all $d$, it is important that we analyze the consequences of Theorem \ref{thm:rmub}. Indeed, it is true that for any $\epsilon \in (0.5,1)$,
%\begin{equation}
%	\label{eq:rmubeps}
%	\mathsf{R}_{(1,\infty)}^{\text{RM}}<\frac{3}{4}(1-\epsilon).
%\end{equation}
%\begin{figure*}[!t]
%	\centering
%	
%	\includegraphics[width=0.9\textwidth]{RMub_achMarkov.png}
%	\caption{Figure shows a comparison between the best numerical information rate achieved using stationary, ergodic first-order Markov input distributions, and the upper bound provided in equation \eqref{eq:rmubeps}, for $\epsilon>0.5$.}
%	\label{fig:rmub}
%\end{figure*}
%Figure \ref{fig:rmub} shows a comparison between the upper bound in equation \eqref{eq:rmubeps}, on the rate achieved by using $(1,\infty)$-RLL subcodes of any capacity-achieving (over the unconstrained BEC) sequence of RM codes, and numerical lower bounds on the capacity without feedback of the $(1,\infty)$-RLL input-constrained BEC. These lower bounds are computed using numerical sampling-based algorithms (see, for example, \cite{Arnold} or \cite{arnk21ncc}), which consider stationary, ergodic, first-order Markov input distributions, and compute their information rates. It is clear from the plots that the upper bound in equation \eqref{eq:rmubeps} is less than the achievable rates of Markov input processes, for $\epsilon>0.5$. Therefore, we conclude that it is not possible to achieve the capacity of the $(1,\infty)$-RLL input-constrained BEC by using $(1,\infty)$-RLL subcodes of RM codes under the lexicographic ordering.
%\begin{remark}
%	While we have proved a pessimistic result under the lexicographic ordering of co-ordinates of the RM code, it is unclear what the best achievable rates are of $(1,\infty)$-RLL subcodes of RM codes obtained by permuting co-ordinates.
%\end{remark}
%We now extend the proof of Theorem \ref{thm:rmub} to general $d$. For ease of notation, we let $z := \left \lceil \log_2(d+1)\right \rceil$. Similar to equation \eqref{eq:rmdecomp}, we note that for any $f\in \mathbb{F}_2[x_1,\ldots,x_m]$, with Eval$(f) \in \text{RM}(m,r)$, it is true that:
%\begin{align}
%	\label{eq:genddecomp}
%f(x_1,\ldots,x_m) &= g_0(x_1,\ldots,x_{m-z})+\notag\\ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \  &\sum_{\substack{{S\subseteq [m-z+1:m],}\\{\ S\neq \emptyset}}} x_Sg_S(x_1,\ldots,x_{m-z}),
%\end{align}
%where we use the notation $x_S$ to denote the monomial $\prod_{i\in S}x_i$, and $g_0$ is such that Eval$(g_0)\in \text{RM}(m-z,r)$ and for any nonempty $S\subseteq [m-z+1:m]$, the polynomials $g_S$ are such that Eval$(g_S)\in \text{RM}(m-z,r-|S|)$.
%
%An important ingredient in the proof for general $d$ is the following lemma, which is a generalization of Lemma \ref{lem:necesscond}:
%\begin{lemma}
%	\label{lem:gend}
%	If a codeword Eval$(f)\in \text{RM}(m,r)$ respects the $(d,\infty)$-RLL constraint, then, supp$(Eval(g_0))\subseteq \text{supp}(\text{Eval}(g_S))$, for all polynomials $g_S$, where $S\subseteq [m-z+1:m]$ is non-empty, and $g_0$ and $g_S$ are as in \eqref{eq:genddecomp}.
%\end{lemma}
%\begin{proof}
%	To this end, we need to show that for any $\mathbf{z}\in \mathbb{F}_2^{m-z}$, it must be that $g_S(\mathbf{z}) = 1$, for all non-empty subsets $S\subseteq [m-z+1:m]$, whenever $g_0(\mathbf{z})=1$, in order for Eval$(f)$ to respect the $(d,\infty)$-RLL constraint. This follows from the simple observation that the Boolean polynomial $\theta(x_{m-z+1},\ldots,x_m):=\prod_{S\subseteq [m-z+1:m]} x_S$ is the only polynomial in the $\left \lceil \log_2(d+1)\right \rceil$ variables $x_{m-z+1},\ldots,x_m$, with the property that $\theta(\mathbf{0}) = 1$ and $\theta(\mathbf{z}) = 0$, for all $\mathbf{z}\neq \mathbf{0}$.
%\end{proof}
%With the lemma above in place, the remainder of the proof of Theorem \ref{thm:rmub} for general $d$ follows similar to the proof when $d=1$. Some salient features are described in the proof below:
%\begin{proof}
%	As earlier, we work with a capacity-achieving (over the unconstrained BEC) sequence of RM codes, $\{\hat{\mathcal{C}}_m = \text{RM}(m,v_m)\}$. 
%	
%	We let $N_w^{(d)}(g_0)$ denote the number of codewords, Eval$(g_S) \in \text{RM}(m-z,r-|S|)$, for non-empty subsets $S\subset [m-z+1:m]$, such that supp$(\text{Eval}(g_0))\subseteq \text{supp}(\text{Eval}(g_S))$, for all $g_S$. We then obtain, similar to equation \eqref{eq:nw}, that:
%	\[
%	N_w^{(d)}(g_0)\leq \text{exp}_2\left((2^z-1)\cdot\left({m-z\choose \leq v_m} - {m-z-u \choose \leq v_m}\right)\right),
%	\]
%	when wt$(\text{Eval}(g_0))\geq 2^{m-z-u}$. Also, we define $\mathscr{R}_{(d,\infty)}^{(m)}$ to be the rate of any $(d,\infty)$-subcode of $\hat{\mathcal{C}}_m$, i.e.,
%	\[
%	\mathscr{R}_{(d,\infty)}^{(m)} = \frac{\log_2(|\mathcal{H}_{(d,\infty)}^{(m)}|)}{2^m},
%	\]
%	where we let $\mathcal{H}_{(d,\infty)}^{(m)}$ denote a $(d,\infty)$-subcode of $\hat{\mathcal{C}}_m$. For ease of reading, we let $\alpha_m^{(d)}:= |\mathcal{H}_{(d,\infty)}^{(m)}|$. Equations \eqref{eq:sub1} and \eqref{eq:sub2} can then be modified to take into account the fact that Eval$(g_0) \in \text{RM}(m-z, v_m)$, and we finally get that:
%	\begin{align}
%		\mathsf{R}_{(d,\infty)}^{\text{RM}} &= \lim_{m\to \infty} \mathscr{R}_{(d,\infty)}^{(m)} \notag\\
%		&< \lim_{m\to \infty} \frac{{m-z \choose \leq v_m}+(2^z-1){m-z-1\choose \leq v_m}}{2^m} \notag\\
%		&= R\cdot \left(\frac{2^z+1}{2^{z+1}}\right), \label{eq:gendappend}
%	\end{align}
%where the complete proof of the equality in \eqref{eq:gendappend} follows from the treatment in Appendix B.
%\end{proof}
